A Decision Procedure for Path Feasibility of String Manipulating Programs with Integer Data Type

Strings are widely used in programs, especially in web applications. Integer data type occurs naturally in string-manipulating programs, and is frequently used to refer to lengths of, or positions in, strings. Analysis and testing of string-manipulating programs can be formulated as the path feasibility problem: given a symbolic execution path, does there exist an assignment to the inputs that yields a concrete execution that realizes this path? Such a problem can naturally be reformulated as a string constraint solving problem. Although state-of-the-art string constraint solvers usually provide support for both string and integer data types, they mainly resort to heuristics without completeness guarantees. In this paper, we propose a decision procedure for a class of string-manipulating programs which includes not only a wide range of string operations such as concatenation, replaceAll, reverse, and finite transducers, but also those involving the integer data-type such as length, indexof, and substring. To the best of our knowledge, this represents one of the most expressive string constraint languages that is currently known to be decidable. Our decision procedure is based on a variant of cost register automata. We implement the decision procedure, giving rise to a new solver OSTRICH+. We evaluate the performance of OSTRICH+ on a wide range of existing and new benchmarks. The experimental results show that OSTRICH+ is the first string decision procedure capable of tackling finite transducers and integer constraints, whilst its overall performance is comparable with the state-of-the-art string constraint solvers.

==> cefa.tex <==
%!TEX root = main.tex


%In this section, we introduce cost-enriched regular languages and recognisable relations, as the extensions of regular languages and recognisable relations, moreover, we investigate the decidability and complexity of a related decision problem, thus laying down the theoretical foundations of the decision procedure in the next section. 

\subsection{Cost-Enriched Regular Languages and Recognisable Relations} \label{sect:ce}

Let $k \in \Nat$ with $k > 0$. A \emph{$k$-cost-enriched string} is $(w, (n_1, \cdots, n_k))$ where $w$ is a string and $n_i \in \intnum$ for all $i \in [k]$. 
A \emph{$k$-cost-enriched language} $L$ is a subset of $\Sigma^* \times \intnum^k$. For our purpose, we identify a ``regular" fragment of cost-enriched languages as follows. 
%Note that all the cost-enriched strings in $L$ are associated with the same number of costs (i.e., $k$).

\begin{definition}[Cost-enriched regular languages]
Let $k \in \Nat$ with $k > 0$. A $k$-cost-enriched language is \emph{regular} (abbreviated as CERL) if it can be accepted by a \emph{cost-enriched finite automaton}. 

A cost-enriched finite automaton (CEFA) $\CEFA$ is a tuple $(Q, \Sigma, R, \delta, I, F)$ where 
\begin{itemize}
\item $Q, \Sigma, I, F$ are defined as in NFAs, 
%
\item $R=(r_1, \cdots, r_k)$ is a vector of (mutually distinct) \emph{cost registers}, 
%
\item $\delta$ is the transition relation which is a finite set of tuples $(q, a, q', \eta)$ where $q, q' \in Q$, $a \in \Sigma$, and %$\eta: R \rightarrow \intnum$ 
$\eta: R \rightarrow \Int$
is a cost register update function. \\
For convenience, we usually write $(q, a, q', \eta) \in \Delta$ as $q \xrightarrow{a, \eta} q'$.
\end{itemize}
%
A \emph{run} of $\CEFA$ on a $k$-cost-enriched string $(a_1 \cdots a_m, (n_1, \cdots,n_k))$ is a  transition sequence $q_0 \xrightarrow{a_1, \eta_1} q_1 \cdots q_{m-1} \xrightarrow{a_m, \eta_m} q_m$ such that $q_0 \in I$ and $n_i = \sum \limits_{1\leq j\leq m}\eta_j(r_i)$ for each $i \in [k]$ (Note that the initial values of cost registers are zero). The run is \emph{accepting} if $q_m \in F$. A $k$-cost-enriched string $(w, (n_1, \cdots,n_k))$ is accepted by $\CEFA$ if there is an accepting run of $\CEFA$ on $(w, (n_1, \cdots,n_k))$. In particular, $(\varepsilon, n)$ is accepted by $\CEFA$ if $n=0$ and $I\cap F \neq \emptyset$.
The $k$-cost-enriched language defined by $\CEFA$, denoted by $\Lang(\CEFA)$, is the set of $k$-cost-enriched strings accepted by $\CEFA$. 
%A cost-enriched language $L \subseteq \Sigma^* \times \intnum^k$ is called a cost-enriched regular language (CERL) if there is a CEFA $\NFA$ such that $L = \Lang(\NFA)$.
\end{definition}
The \emph{size} of a CEFA $\CEFA=(Q, \Sigma, R, \delta, I, F)$, denoted by $|\CEFA|$, is defined as the sum of the sizes of its transitions, where the size of each transition $(q, a, q', \eta)$ is $\sum \limits_{r \in R} \lceil \log_2 (|\eta(r)|) \rceil +3$. Note here  the integer constants in $\CEFA$ are encoded in binary.

\begin{remark}
CEFAs can be seen as a variant of Cost Register Automata \cite{RLJ+13}, by admitting nondeterminism and discarding partial final cost functions. CEFAs are also closely related to monotonic counter machines \cite{LB16}. The main difference is that CEFAs discard guards in transitions and allow binary-encoded integers in cost updates, while monotonic counter machines allow guards in transitions but restrict the cost updates to being monotonic and unary, i.e. $0,1$ only. Moreover, we explicitly define CEFAs as language acceptors for  cost-enriched languages.
\end{remark}

\begin{example}[CEFA for $\length$]\label{exm:len}
The string function $\length$ can be captured by CEFAs. For any NFA $\NFA=(Q, \Sigma,  \delta, I, F)$, it is not difficult to see that the cost-enriched language $\{(w, \length(w)) \mid w\in \Lang(\NFA)\}$ is accepted by a CEFA, i.e., 
$(Q, \Sigma, (r_1), \delta', I, F)$  %$Q =I=F= \{q_0\}$, $R=(r_1)$, and 
such that for each $(q, a, q')\in \delta$, we let $(q, a, q', \eta)\in \delta'$, where $\eta(r_1) = 1$. 

For later use, we identify a special $\CEFA_{\rm len}= (\{q_0\}, \Sigma, (r_1), \{(q_0, a, q_0, \eta) \mid \eta(r_1) = 1\}, \{q_0\}, \{q_0\})$. In other words, $\CEFA_{\rm len}$ accepts $\{(w, \length(w)) \mid w\in \Sigma^*\}$.
%
%
%to denote the CEFA $(Q, \Sigma, (r_1), \delta', I, F)$ for the special NFA $\NFA$ such that $\Lang(\NFA)=\Sigma^*$, specifically, $\NFA_{\rm len} = (\{q_0\}, \Sigma, (r_1), \{(q_0, a, q_0, \eta) \mid \eta(r_1) = 1\}, \{q_0\}, \{q_0\})$.
%\tl{it is a bit vague; you mean for any RE $e$,  is a cerl?}
\end{example}

We can show that the function $\indexof_v(\cdot, \cdot)$ can be captured by CEFAs as well, in the sense that, for any NFA $\NFA$ and constant string $v$, we can construct a CEFA %$\CEFA'$ such that 
accepting $\left\{(w, (n, \indexof_v(w, n)))\mid w\in \Lang(\NFA), n \le \indexof_v(w, n) < |w| \right\}$. %$R(\CEFA')=(r_1,r_2)$ and $\Lang(\CEFA')=\{(w, (n, \indexof_v(w, n)))\mid w\in \Lang(\NFA) \}$. 
The construction is slightly technical and can be found in Appendix, Section~\ref{appendix:cefa_indexof}.

For convenience, we use $\CEFA_{\indexof_v}$ which accepts $\{(w, (n, \indexof_v(w, n)))\mid w\in \Sigma^*, n \le \indexof_v(w, n) < |w| \}$. %to denote the constructed CEFA $\CEFA'$ for the special NFA $\NFA$ such that $\Lang(\NFA)=\Sigma^*$. 
Note that $\CEFA_{\indexof_v}$ does not model the corner cases in the semantics of $\indexof_v$, for instance, $\indexof_v(w, n) = -1$ if $v$ does not occur after the position $n$ in $w$.
In the sequel, we will give an example of the construction of $\CEFA_{\indexof_v}$ for the special case that $v$ is a single letter.  

\begin{example}[CEFA for $\indexof_a$]\label{exm:indexof}
Let $a \in \Sigma$. Then  $\CEFA_{\indexof_a} = (\{(q_0, q_1, q_2)\}, \Sigma, (r_1,r_2), \delta_{\indexof_a}, \{q_0\}, \{q_2\})$, where $\delta_{\indexof_a}$ comprises the tuples
\begin{itemize}
\item $(q_0, b, q_0, \eta)$ such that $b \in \Sigma$, $\eta(r_1)=1$, $\eta(r_2)=1$,
%
\item $(q_0, b, q_1, \eta)$ such that $b \in \Sigma$, $\eta(r_1)=0$, $\eta(r_2) = 1$,
%
\item $(q_0, a, q_2, \eta)$ such that $\eta(r_1)=0$, $\eta(r_2) = 0$,
%
\item $(q_1, b, q_1, \eta)$ such that $b \in \Sigma \setminus \{a\}$, $\eta(r_1)=0$, $\eta(r_2)=1$,
%
\item $(q_1, a, q_2, \eta)$ such that $\eta(r_1)=0$, $\eta(r_2)=0$,
%
\item $(q_2, b, q_2, \eta)$ such that $b \in \Sigma$, $\eta(r_1)=0$, $\eta(r_2)=0$.
\end{itemize}
Intuitively, $r_1$ corresponds to the starting position $i$ of $\indexof_a(x, i)$, $r_2$ corresponds to the output of $\indexof_a(x, i)$, $q_0$ specifies that the current position is before $i$, $q_1$ specifies that the current position is after $i$, while $a$ has not occurred yet, and $q_2$ specifies that $a$ has occurred after $i$. 
\end{example}


Given two CEFAs $\CEFA_1 = ( Q_1, \Sigma, R_1, \delta_1, I_1, F_1)$ and $\CEFA_2 = (Q_2, \Sigma, \delta_2, R_2, I_2, F_2)$ with $R_1 \cap R_2 = \emptyset$ (where %the notation is abused a bit, viewing 
$R_1$ and $R_2$ are treated as sets), the product of $\CEFA_1$ and $\CEFA_2$, denoted by $\CEFA_1 \times \CEFA_2$, is defined as $(Q_1 \times Q_2, \Sigma, R_1 \cup R_2, \delta, I_1 \times I_2, F_1 \times F_2)$, where $\delta$ comprises the tuples $((q_1, q_2), \sigma, (q'_1, q'_2), \eta)$ such that $(q_1, \sigma, q'_1, \eta_1) \in \delta_1$, $(q_2, \sigma, q'_2, \eta_2) \in \delta_2$, and $\eta = \eta_1\cup \eta_2$.  %for some $\eta_1, \eta_2$.


For a CEFA $\CEFA$, we use $R(\CEFA)$ to denote the vector of cost registers occurring in $\CEFA$. %Note that cost registers of $\CEFA$ are simply integer variables to store costs in $\CEFA$.
%Moreover, for a CEFA $\NFA$ and 
Suppose $\CEFA$ is  CEFA with $R(\CEFA)=(r_1,\cdots, r_k)$ and $\vec{i} = (i_1,\cdots, i_k)$ is a vector of mutually distinct integer variables such that $R(\NFA) \cap \vec{i} = \emptyset$. We use $\CEFA[\vec{i}/R(\CEFA)]$ to denote the CEFA obtained from $\CEFA$ by simultaneously replacing $r_j$ with $i_j$ for $j \in [k]$. 

\smallskip

%Let $(k_1,\cdots, k_l) \in \Nat^l$ with $k_j > 0$ for every $j \in [l]$. A  $(k_1,\cdots, k_l)$-cost-enriched relation $\cR$ is a subset of $(\Sigma^* \times \intnum^{k_1}) \times \cdots (\Sigma^* \times \intnum^{k_l})$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}[Cost-enriched recognisable relations]
Let $(k_1,\cdots, k_l) \in \Nat^l$ with $k_j > 0$ for every $j \in [l]$. A cost-enriched recognisable relation (CERR)  $\cR \subseteq (\Sigma^* \times \intnum^{k_1}) \times \cdots  \times (\Sigma^* \times \intnum^{k_l})$ is a finite union of products of CERLs. Formally,
$\cR = \bigcup \limits_{i=1}^n L_{i,1 } \times \cdots \times L_{i, l}$, 
	where for every $j \in [l]$, $L_{i,j} \subseteq \Sigma^* \times \intnum^{k_j}$ is a CERL. 
	A CEFA representation of $\cR$ is a collection of CEFA tuples $(\CEFA_{i,1}, \cdots, \CEFA_{i,l})_{i \in [n]}$ such that $\Lang(\CEFA_{i,j}) = L_{i,j}$ for every $i \in [n]$ and $j \in [l]$.
\end{definition}

\begin{example}\label{exm:CERR}
The relation 
\[\cR=\left\{((w_1, |w_1|), (w_2, |w_2|)) \mid  w_1 \in \Lang((aa)^*), w_2 \in \Lang(b(bb)^*), |w_1|+|w_2| \ge 2\right\}\] 
is a CERR since 
$\cR = L_{1,1} \times L_{1,2} \cup L_{2,1} \times L_{2,2}$, where $L_{1,1}=\{(w_1, |w_1|) \mid w_1 \in \Lang((aa)^*)\}$, $L_{1,2}=\{(w_2, |w_2|) \mid  w_2 \in \Lang(bbb(bb)^*)\}$, $L_{2,1}=\{(w_1, |w_1|) \mid w_1 \in \Lang(aa(aa)^*)\}$, and $L_{2,2}=\{(w_2, |w_2|) \mid  w_2 \in \Lang(b(bb)^*)\}$.
%\begin{itemize}
%\item $L_{1,1}=\{(w_1, |w_1|) \mid w_1 \in \Lang((aa)^*)\}$, 
%\item $L_{1,2}=\{(w_2, |w_2|) \mid  w_2 \in \Lang(bbb(bb)^*)\}$ , 
%\item $L_{2,1}=\{(w_1, |w_1|) \mid w_1 \in \Lang(aa(aa)^*)\}$,  and
%\item $L_{2,2}=\{(w_2, |w_2|) \mid  w_2 \in \Lang(b(bb)^*)\}$. 
%\end{itemize}
Note that $L_{i,j}$ for $i,j\in[2]$ are CERLs, with corresponding CEFAs $\CEFA_{i,j}$ by  Example~\ref{exm:len}. It follows that %Moreover, 
$(\CEFA_{i,1}, \CEFA_{i,2})_{i \in [2]}$ gives a CEFA representation of $\cR$. %, where 
%\tl{to be simplified.}
%\begin{itemize}
%\item  $\CEFA_{1,1} = (\{p_0, p_1\}, \{a,b\}, (r_{1}), \delta_{1,1}, \{p_0\}, \{p_0\})$ defines $L_{1,1}$, such that $\delta_{1,1}= \{(p_0, a, p_1,\eta_1)$, $(p_1, a, p_0, \eta_1)\}$, with $\eta_1(r_{1})=1$,
%%
%\item $\CEFA_{1,2}=(\{q_0,q_1,q_2\}, \{a,b\}, (r_{2}), \delta_{1,2}, \{q_0\}, \{q_1\})$ defines $L_{1,2}$, such that $\delta_{1,2}=\{(q_0, b, q_1,\eta_2), (q_1, b, q_2, \eta_2), (q_2, b, q_1,\eta_2)\}$, with $\eta_2(r_{2})=1$,
%%
%\item $\CEFA_{2,1} = (\{p_0, p_1,p_2, p_3\}, \{a,b\}, (r_{1}), \delta_{2,1}, \{p_0\}, \{p_2\})$ defines $L_{2,1}$, such that $\delta_{2,1} = \{(p_0, a, p_1, \eta_1), (p_1, a, p_2, \eta_1), (p_2, a, p_3, \eta_1), (p_3, a, p_2, \eta_1)\}$, with $\eta_1(r_{1})=1$, and
%%
%\item $\CEFA_{2,2}=(\{q_0,q_1,q_2\}, \{a,b\}, (r_{2}), \delta_{2,2}, \{q_1\})$ defines $L_{2,2}$, such that $\delta_{2,2}= (q_0, b, q_1,\eta_2), (q_1, b, q_2, \eta_2), (q_2, b, q_1,\eta_2)\}$, with $\eta_2(r_{2})=1$.
%\end{itemize}
\end{example}

%\subsection{Satisfiability of Linear Integer Arithmetic Formula with respect to CEFAs}
%
%In the sequel, we consider a decision problem for CEFAs which will be used for the decision procedure of the path feasibility problem for {\slint} in the next section.
%
%\begin{definition}[{\lasat} Problem]\label{def-la-sat-cefa}
%	The satisfiability problem of LIA formulas w.r.t. CEFAs (abbreviated as {\lasat} problem) is defined as follows.
%	
%	\textbf{Input}: a given quantifier-free LIA formula $\phi$ and CEFAs $\CEFA_1,\cdots,\CEFA_m$, such that $\CEFA_i=(Q_i, \Sigma, R_i, \delta_i, I_i, F_i)$ for every $i\in [m]$, 
%  $R_i \cap R_j = \emptyset$ for every $1 \le i < j \le m$, and
% the free variables of $\phi$ are from $\bigcup_{i\in [m]} R_i$, 
% 
%Decide whether %$\phi$ is satisfiable w.r.t. $\CEFA_1, \cdots, \CEFA_m$, namely, whether 
%there are an assignment function $\theta: \bigcup \limits_{i \in [m]} R_i \rightarrow \Int$ and strings $w_1, \cdots, w_m$  
%	such that  $\phi[(\theta(R_i)/R_i)_{i \in [m]}]$ hold and $(w_i, \theta(R_i)) \in \Lang(\NFA_i)$ for every $i \in [m]$.
%\end{definition}
%%Note that in Definition~\ref{def-la-sat-cefa}, registers in $\NFA_i$'s may intersect. 
%
%\begin{example}
%Let $\phi \equiv r_1 = r_2$ and $\CEFA_{1,1}, \CEFA_{1,2}$ be two CEFAs in Example~\ref{exm:CERR} defining $L_{1,1}, L_{1,2}$ respectively. (Recall that $R(\CEFA_{1,1})=(r_1)$ and $R(\CEFA_{1,2})=(r_2)$.) Then it is easy to see that $\phi$ is unsatisfiable w.r.t. $\CEFA_{1,1}$ and $\CEFA_{1,2}$, since for each $(w_1, n_1) \in L_{1,1}$, $n_1$ must be even, while for each $(w_2, n_2) \in L_{1,2}$, $n_2$ must be odd. Hence $n_1$ and $n_2$ cannot be equal.
%\end{example}
%
%\begin{theorem}\label{thm-la-sat-cefa}
%	The {\lasat} problem is NP-complete.
%\end{theorem}
%The proof is given in Appendix, Section~\ref{appendix:thm-la-sat-cefa}.


==> runexmp.tex <==
%!TEX root = main.tex
 
\section{Running example} \label{exmp:running}
We use the following JavaScript program as the running example,
%which demonstrates the use of string functions coupled with integer data type as well as path feasibility of string-manipulating programs.
which defines a function {\urlxsssanitise} for sanitising URLs. A typical URL consists of a hierarchical sequence of components commonly referred to as protocol, host, path, query, and fragment. For instance, in ``\url{http://www.example.com/some/abc.html?name=john#print}'', the protocol is ``{\tt http}'', the host is ``{\tt www.example.com}'', the path is ``{\tt /some/abc.html}'', the query is ``{\tt name=john}'' (preceded by $?$), and the fragment is ``{\tt print}'' (preceded by $\#$). Both the query and the fragment could be empty in a URL. The aim of {\urlxsssanitise} is to mitigate \emph{URL reflection attacks} \cite{url-reflect}, by filtering out the dangerous substring ``\url{script}'' from the query and fragment components of  the input URL. URL reflection attacks are a type of cross-site-scripting (XSS) attacks that do not rely on saving malicious code in database, but rather on hiding it in the query or fragment component of URLs, e.g., ``\url{http://www.example.com/some/abc.html?name=<script>alert('xss!');</script>}''.

%\begin{example}
{\small
\begin{minted}[linenos]{javascript}
function urlXssSanitise(url) {
    var prothostpath='', querfrag = '';
    url = url.trim();
    var qmarkpos = url.indexof('?'), sharppos = url.indexof('#');
    if(qmarkpos >= 0) 
    {   prothostpath = url.substr(0, qmarkpos);
        querfrag = url.substr(qmarkpos); }
    else if(sharppos >= 0)
    {   prothostpath = url.substr(0, sharppos);
        querfrag = url.substr(sharppos); }
    else prothostpath = url;
    querfrag = querfrag.replace(/script/g, '');
    url = prothostpath.concat(querfrag);
    return url;
}
\end{minted}
}
%\end{example}

\noindent Note that {\urlxsssanitise} uses the JavaScript sanitisation operation $\sf trim$ that removes whitespace from both ends of a string, which can be conveniently modelled by finite-state transducers. Two string functions involving the integer data type, namely, $\sf indexof$ and $\sf substr$ ($\indexof$ and $\substring$ in this paper), as well as concatenation and $\sf replace$ (with the `g'---global---flag, called $\replaceall$ in this paper), are present. 

%$\footnote{$\sf replace$ with the g flag in Javascript corresponds to the $\replaceall$ function in this paper.}

% \in [\backslash w | \backslash x2E]^*$
%We expect that the returned value of the ``host'' variable contains only the alphanumeric symbols as well as the dot symbol, but actually this is not the case. This question can be reduced to solving the path feasibility problem of the following program of the SSA (single static assignment) form.

The program analysis is to ascertain whether {\urlxsssanitise} indeed works, namely, after applying {\urlxsssanitise} to the input URL, ``\url{script}'' does not appear.  This problem can be reduced to checking whether there is an execution path of {\urlxsssanitise} that produces an output such that its query or fragment component contains occurrences of ``\url{script}''. For instance, assuming  the ``if'' branch is executed, %first execution path of {\urlxsssanitise} is chosen, then the problem is reduced to 
we will need to solve the path feasibility of the following JavaScript program in single static assignment (SSA) form,

{\small
\begin{minted}{javascript}
    prothostpath =''; querfrag = '';
    url1 = url.trim(); qmarkpos = url1.indexof('?');
    sharppos = url1.indexof('#'); assert(qmarkpos >= 0); 
    prothostpath1 = url1.substr(0, qmarkpos);
    querfrag1 = url1.substr(qmarkpos);
    querfrag2 = querfrag1.replace(/script/g, '');
    url2 = prothostpath1.concat(querfrag2);
    assert(/script/.test(querfrag2))
\end{minted}
}

\vspace*{-0.5ex}
\noindent where the $\ASSERT{cond}$ statement checks that the condition $cond$ is satisfied. As one will see later, this can be directly encoded in our constraint language (cf.\ Section~\ref{sec:logic}) and handled by the decision procedure (cf. Section~\ref{sec:dec}). 
%Back to Example~\ref{exmp:running}, 
Our solver  {\ostrich}+ can solve the path feasibility of the aforementioned 
SSA program in several seconds. This is far from trivial since %the program contains not only 
the solver needs to tackle complex string functions such as {\tt trim()} (modelled as finite transducers) and {\tt replaceAll}, %but also those involving the integer data type, namely 
as well as %$\length$, 
$\indexof$  and $\substring$, which is beyond the scope of other existing decision procedures.  
%\qed
%\end{example}

